$\alpha$-Flow: A Unified Framework for Continuous-State Discrete Flow Matching Models

Recent efforts have extended the flow-matching framework to discrete generative modeling. One strand of models directly works with the continuous probabilities instead of discrete tokens, which we colloquially refer to as Continuous-State Discrete Flow Matching (CS-DFM). Existing CS-DFM models differ significantly in their representations and geometric assumptions. This work presents a unified framework for CS-DFM models, under which the existing variants can be understood as operating on different $\alpha$-representations of probabilities. Building upon the theory of information geometry, we introduce $\alpha$-Flow, a family of CS-DFM models that adheres to the canonical $\alpha$-geometry of the statistical manifold, and demonstrate its optimality in minimizing the generalized kinetic energy. Theoretically, we show that the flow matching loss for $\alpha$-flow establishes a unified variational bound for the discrete negative log-likelihood. We comprehensively evaluate different instantiations of $\alpha$-flow on various discrete generation domains to demonstrate their effectiveness in discrete generative modeling, including intermediate values whose geometries have never been explored before. $\alpha$-flow significantly outperforms its discrete-state counterpart in image and protein sequence generation and better captures the entropy in language modeling.

==> secs/3_method_alt.tex <==
\section{Method}
To leverage the continuous Riemannian flow matching framework, CS-DFM models should deduce a geometric structure on the manifold of categorical distributions. In differential geometry, a metric $g$ that defines an inner product for vector fields and the affine connection $\nabla$ that allows for differentiation of the nearby vector fields generates a Riemannian structure. For statistical manifold, the Fisher information metric is the canonical metric. On the other hand, the different definitions of affine connections allow us to equip the same manifold with different geometries, allowing for a unified view to analyze the geodesics on the statistical manifold. We will demonstrate that all the variants of the current CS-DFM models can be unified under the $\alpha$-\emph{geometry} of the statistical manifold.

\subsection{$\alpha$-Geometry on Statistical Manifold}
\begin{definition}[$\alpha$-Representation]
For $\alpha\in[-1,1]$, the $\alpha$-\emph{representation} of a positive measure $m\in\mathcal{M}_+$ is defined by the embedding $\pi^{(\alpha)}:\mathcal{M}_+\hookrightarrow\mathbb{R}_+^N$:
\begin{equation}
    m\mapsto x=\frac{2}{1-\alpha}\left(m^\frac{1-\alpha}{2}-1\right)=p(m^{1/p}-1)\label{eqn:mapping}
\end{equation}
where $p=2/(1-\alpha)$. Specifically, for $\alpha=1$, taking the limit, we get $\pi^{(1)}:m\mapsto\log m$.
\end{definition}

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figs/representation.png}
    \caption{$\alpha$-representations of a Bernoulli distribution.}
    \label{fig:representation}
\end{figure}

The $\alpha$-representation conincides with the Tsallis $q$-logarithm $\log_q \mu$ where $q=(1+\alpha)/2$. The $\alpha$-\emph{geometry} for positive measures can be understood as operating on such $\alpha$-representation with a flat geometry $x_t=(1-t)x_0+tx_1$, which is equivalent to:
\begin{equation}
    m_t^{1/p}:=\gamma^{(\alpha)}_{m_0,m_1}(t)^{1/p}=(1-t)m_0^{1/p}+tm_1^{1/p}
\end{equation}
The geodesic $\gamma^{(\alpha)}_{m_0,m_1}$ is called $\alpha$-\emph{geodesic}.
For probability measure $\mu\in\mathcal{P}_+\subseteq\mathcal{M}_+$, the $\alpha$-representation lies on the (translated) positive orthant of the $L_p$ sphere with radius $p$. Mathematical literature \cite{morozova1991markov,ay2017information} demonstrated that the $\alpha$-geodesics adopt the following general form:
\begin{equation}
     \gamma^{(\alpha)}_{\mu,\nu}(t)^{1/p}=\frac{(1-\tau_{\mu,\nu}(t))\mu^{1/p}+\tau_{\mu,\nu}(t)\nu^{1/p}}{\|(1-\tau_{\mu,\nu}(t))\mu^{1/p}+\tau_{\mu,\nu}(t)\nu^{1/p}\|_p}
\end{equation}
where $\tau_{\mu,\nu}$ is an appropriate reparameterization of time with $\tau_{\mu,\nu}(0)=0,\tau_{\mu,\nu}(1)=1$. Additionally, the exponential map and logarithm map can be calculated as:
\begin{align}
    \left(\exp^{(\alpha)}_\mu(a)\right)^{1/p}&=\frac{\mu^{1/p}+\frac{\tau_{\mu,a}(t)\mu^{1/p}}{p\mu}a}{\|\mu^{1/p}+\frac{\tau_{\mu,a}(t)\mu^{1/p}}{p\mu}a\|_p},\label{eqn:ori_exp}\\
    \log^{(\alpha)}_\mu(\nu)&=\dot\tau_{\mu,\nu}(0) P_\mu\left(\mu\pi^{(\alpha)}(\nu/\mu)\right)\label{eqn:ori_log}
\end{align}
where $P_\mu(w)=w-\mu\sum_j w_j$ denotes the orthogonal projection onto the tangent space $T_\mu\mathcal{P}$ and $\tau_{\mu,a}$ is the compatible reparameterization of time with $\tau_{\mu,a}(0)=0,\dot\tau_{\mu,a}(1)=1$. In this way, the probability paths follow different $\alpha$-geodesics on the statistical manifold, leading to different Riemannian geometries on which the flow-matching loss can be written as
\begin{equation}
    \mathcal{L}^{(\alpha)}=\mathbb{E}_{t,p_0(\mu),q(\mu)}\|v_\theta(\gamma^{(\alpha)}(t),t)-\dot{\gamma}^{(\alpha)}(t)\|_g^2 \label{eqn:loss}
\end{equation}
where $\gamma^{(\alpha)}(t)$ denotes the $\alpha$-geodesic from $\mu_0$ to $\mu_1$. In this way, this unified framework $\alpha$-\emph{geodesic flow} equips the statistical manifold with different Riemannian geometries for generative modeling. The different exponential maps and interpolations are demonstrated in Fig.\ref{fig:geodesic}.

\begin{figure}
    \centering
    \includegraphics[width=0.49\linewidth]{figs/exponential.png}
    \includegraphics[width=0.49\linewidth]{figs/interpolation.png}
    \caption{$\alpha$-geodesics defined by the exponential map (\textbf{left}) of the same base point and vector field, and the interpolation (\textbf{right}) between two fixed points on the 2-simplex.}
    \label{fig:geodesic}
\end{figure}

Generally, a neural net can be directly trained to regress the vector field above. Nonetheless, the division by $\mu$ may lead to numerical issues. Similar to previous work \cite{cheng2024categorical,davis2024fisher}, we can also parameterize the vector field on the mapped manifold of the $L_p$ sphere to avoid such issues. Consider the vector field mapping by taking the derivative with respect to $t$ on both sides of Eq.\ref{eqn:mapping}:
\begin{equation}
    u_t:=\frac{\diff}{\diff t}x_t=\frac{\mu_t^{1/p}}{\mu_t} a_t=\frac{1}{\mu_t^{(1+\alpha)/2}}a_t. \label{eqn:vf_mapping}
\end{equation}
The transformed vector field $u$ lies in the tangent space $T_x S_p$ of the $L_p$ sphere at $x={\pi}^{(\alpha)}(\mu)$. In this way, the exponential and logarithm maps have simplified forms as
\begin{align}
    &\widetilde{\exp}^{(\alpha)}_x(u)=p\left(\frac{x+p+\tau_{\mu,a}(t)u}{\|x+p+\tau_{\mu,a}(t)u\|_p}-1\right),\label{eqn:mapped_exp} \\ 
    &\widetilde{\log}^{(\alpha)}_x(y)=\dot\tau_{\mu,\nu}(0)P^{(\alpha)}_\mu(y-x)\label{eqn:mapped_log}
\end{align}
where $P^{(\alpha)}_\mu(w)=w-\mu^{(1-\alpha)/2}\sum_j\mu^{(1+\alpha)/2}_jw_j$ denotes the orthogonal projection to the tangent space $T_x S_p$.
The original Riemannian norm $\|a\|_g^2=\sum_{i}a_i^2/\mu_i$ can be substituted with 
\begin{equation}
    \|u\|_\alpha^2:=\|a\|_g^2=\sum_{i=1}^n u_i^2\mu_i^{\alpha} . \label{eqn:mapped_norm}
\end{equation}
This transform allows us to parameterize the vector field on the $L_p$ sphere with 
\begin{equation}
    v_\theta(x_t,t):=P^{(\alpha)}_{\mu_t}\big(\tilde{v}_\theta(x_t,t)\big)\label{eqn:proj_vf}
\end{equation}
where $\tilde{v}_\theta$ is the unconstrained predictor. In this way, the final vector field is guaranteed to lie in the tangent space $TS_p$, and the model is expected to learn the marginalized linear difference of the $\alpha$-representations of $y-x$. A further simplification that discards the scaling and translation for $\alpha\ne 1$ is discussed in Appendix \ref{}. 
Nonetheless, in the following discussion of the theoretical properties of $\alpha$-geodesic flow, we will stick with the original exponential and logarithm maps in Eq.\ref{eqn:ori_exp} and \ref{eqn:ori_log}, as the change of parameterization does not impact these theoretical results.


\begin{algorithm}[ht]
\caption{Training $\alpha$-geodesic flow}\label{alg:train}
\begin{algorithmic}[1]
\WHILE{not converged}
    \STATE Sample $\mu_1\sim q(\mu),\mu_0\sim p_0(\mu)$.
    \STATE Apply $x_1=\pi^{(\alpha)}(\mu_1),x_0=\pi^{(\alpha)}(\mu_0)$ in Eq.\ref{eqn:mapping}.
    \STATE Sample $t\sim U[0,1]$ and calculate the mapped geodesic $x_t=\widetilde{\exp}_{x_0}^{(\alpha)}\big(t\widetilde{\log}_{x_0}^{(\alpha)}(x_1)\big)$ using Eq.\ref{eqn:mapped_exp}, \ref{eqn:mapped_log}.
    \STATE Calculate the vector field $u_t=\widetilde{\log}_{x_t}^{(\alpha)}(x_1)/(1-t)$.
    \STATE Optimize the loss $\|v_\theta(x_t,t)-u_t\|_\alpha^2$ using Eq.\ref{eqn:mapped_norm}.
\ENDWHILE
\end{algorithmic}
\end{algorithm}


\subsection{Variational Bound for Negative Log-Likelihood}
The conditional flow matching framework enjoys the exact likelihood calculation. However, as discussed in previous work \cite{cheng2024categorical}, such a likelihood is with respect to the distribution over categorical distributions $p(\mu)$ and, therefore, non-comparable to the discrete categorical likelihood of $\mu$. In this subsection, we demonstrate for the first time that, similar to masked diffusion models, a variational bound can be established for the discrete negative log-likelihood (NLL) for all $\alpha$-geodesic flows.

\begin{theorem}[Negative ELBO]\label{thm:elbo}
For all $\alpha\in[-1,1]$, the loss $\mathcal{L}^{(\alpha)}$ establishes a negative evidence lower bound (ELBO) for the discrete negative log-likelihood:
\begin{equation}
    -\log p(\delta)\le \frac{1}{2}\mathbb{E}_{t,p_0(\mu)}\|v_\theta(\gamma^{(\alpha)}(t),t)-\dot{\gamma}^{(\alpha)}(t)\|_g^2+C
\end{equation}
where $\delta$ is the target categorical distribution, $\gamma^{(\alpha)}$ is the $\alpha$-geodesic from $\mu_0$ to $\delta$, and $C$ is a constant.
\end{theorem}
First, we introduce an important proposition regarding the property of KL-divergence.
\begin{proposition}\label{prop:div_taylor}
For $\mu\in\mathcal{P}_+$, the following expansion holds
\begin{equation}
D_\text{\rm KL}(\mu\|\mu+\mathrm{d}\mu)=\frac{1}{2}\|\mathrm{d}\mu\|_g^2 +o(\|\mathrm{d}\mu\|_g^2)
\end{equation}
\end{proposition}
This proposition established the connection between KL-divergence and the Fisher information metric, which can be directly verified by taking the partial derivatives with respect to probabilities. We can prove Theorem~\ref{thm:elbo} as follows.
\begin{proof}
First, we noted the standard ELBO formulation for the diffusion process. The variational bound can be established as
\begin{align}
    \mathcal{L}&=\mathbb{E}_{p_0(\mu_0)}\Big[-\log p_\theta(\delta|\mu_1)\\
    &+\int_0^1 \frac{1}{\mathrm{d}t}D_\text{KL}\big(q(\mu_{t+\mathrm{d} t}|\mu_t,\delta)\|p_\theta(\mu_{t+\mathrm{d}t}|\mu_t)\big)\\
    &+D_\text{KL}\left(q(\mu_0|\delta)\|p_\theta(\mu_0)\right)\Big] %\ge -\log p(\delta)
\end{align}
where $q$ denotes the categorical distribution generated by the true denoising process and $p_\theta$ denotes the predicted categorical distribution (in the infinitesimal sense). The three components are also known as the reconstruction, diffusion, and prior losses, respectively.
For $\alpha$-geodesic flow, we have $\mu_1\equiv\delta$ as $\tau_{\mu,\nu}(1)=1$ in the interpolation. Therefore, the reconstruction loss is always 0.
As $p_0(\mu)$ is independent of $\delta$, the prior loss is a non-negative constant $C$ that does not rely on the model.

For an infinitesimal diffusion step $\diff t$, using Proposition~\ref{prop:div_taylor}, the integrant of $D_\text{KL}$ can be approximated as
\begin{align}
    &\quad D_\text{KL}\big(q(\mu_{t+\mathrm{d}t}|\mu_t,\delta)\|p_\theta(\mu_{t+\mathrm{d}t}|\mu_t)\big)\\
    &\approx D_\text{KL}\left(\mu_t+\dot{\gamma}^{(\alpha)}(t)\diff t\|\mu_t+v_\theta(\mu_t,t)\diff t\right)\\
    &\approx\frac{1}{2}\|\dot{\gamma}^{(\alpha)}(t)-v_\theta(\mu_t,t)\|_g^2\diff t^2.
\end{align}
In the first equation, we use the first-order Taylor expansion of the exponential map $\exp^{(\alpha)}_\mu(a)\approx\mu+a$. Therefore, integrating over $t$, we get
\begin{equation}
    \mathcal{L}=\frac{1}{2}\int_0^1 \|\dot{\gamma}^{(\alpha)}(t)-v_\theta(\mu_t,t)\|_g^2 \diff t+C=\frac{1}{2}\mathcal{L}^{(\alpha)}+C
\end{equation}
\end{proof}

In this way, when optimizing the loss in Eq.\ref{eqn:loss}, it is equivalent to optimizing the negative ELBO for the discrete likelihood. It is also worth noting that such a variational bound is not directly comparable to those in masked diffusion models whose prior loss is always zero due to the deterministic start point from masks. However, it is still helpful as the loss gradient is essentially the same.

\subsection{Optimality of $\alpha$-Geodesic Flow}
\begin{definition}[$\alpha$-Divergence]
The following function $D^{(\alpha)}:\mathcal{P}_+\times \mathcal{P}_+\to\mathbb{R}_+$ is called the $\alpha$-\emph{divergence}:
\begin{equation}
    D^{(\alpha)}(\mu\|\nu):=\frac{4}{1-\alpha^2}\sum_{i\in\mathcal{X}}\nu_i^{\frac{1+\alpha}{2}}\mu_i^{\frac{1-\alpha}{2}} .
\end{equation}
\end{definition}
The $\alpha$-divergence can be naturally continued at $\alpha=\pm 1$ by taking the limit to obtain $D^{(-1)}(\mu\|\nu)=D_\text{KL}(\mu\|\nu)$ and $D^{(1)}(\mu\|\nu)=D_\text{KL}(\nu\|\mu)$. 
% A similar property holds for all $\alpha$-divergence:
% \begin{proposition}
% For $\mu\in\mathcal{P}_+$, for $\alpha\in[-1,1]$, we have
% \begin{equation}
%     D^{(\alpha)}(\mu\|\mu+\mathrm{d}\mu)=\frac{1}{2}\|\mathrm{d}\mu\|_g^2 +o(\|\mathrm{d}\mu\|_g^2) .
% \end{equation} 
% \end{proposition}
% This proposition is a direct generalization of KL-divergence, a special case of $\alpha=-1$. 

\begin{proposition}[\citet{ay2017information}, Sec.2.7.3]\label{prop:gradient}
\begin{equation}
    \log^{(\alpha)}_\mu \nu = \dot\tau_{\mu,\nu}(0)\left(-\grad_\mu D^{(-\alpha)}(\cdot\|\nu)\right) .
\end{equation} 
\end{proposition}
In other words, the vector field direction along the $\alpha$-geodesics coincides with the projection of the negative gradient of the $(-\alpha)$-divergence, the steepest direction of decreasing $(-\alpha)$-divergence.
For general non-Levi-Civita connections, the local length-minimizing properties of the geodesics are no longer valid. However, a generalization of the statement is available:
\begin{theorem}[local optimality, \citet{bauer2024p}, Corollary 3.11]\label{thm:local_optim}
The $\alpha$-geodesic $\gamma^{(\alpha)}$ describes locally minimizing curves of the (local) $\alpha$-\emph{energy} defined as
\begin{equation}
    E^{(\alpha)}(\mu):=\frac{1}{p}\int_0^1 F^p(\gamma,\dot{\gamma}) \diff t
\end{equation}
for any locally defined smooth curve $\gamma$ starting at $\mu$, where $F(\gamma,\dot{\gamma})$ is the Finsler metric
\begin{equation}
    F(\mu,a):=\left(\sum_{i=1}^n\left|\frac{a_i}{\mu_i}\right|^p\mu_i\right)^{1/p} .
\end{equation}
\end{theorem}

As a special case of the Levi-Civita connection when $\alpha=0,p=2$, the Finsler metric coincides with the Fisher information metric, and we obtain:
\begin{corollary}
The 0-geodesic locally minimizes the curve length and the kinetic energy $\frac{1}{2}\int_0^1\|\dot{\gamma}\|_g^2\diff t$.
\end{corollary}

Furthermore, as we confine ourselves to the positive orthant of the $L_p$ sphere, the geodesic is unique (\citet{bauer2024p}, Theorem 4.2), leading to global optimality:
% \begin{proposition}
% The $\alpha$-divergence is the \emph{canonical divergence} of the Riemannian structure $(g,\nabla^{(\alpha)})$, i.e., the following holds:
% \begin{equation}
%     D^{(\alpha)}(\mu\|\nu)=\int_0^1 t\|\dot{\gamma}_{\mu,\nu}(t)\|^2_g \diff t=\int_0^1 (1-t)\|\dot{\gamma}_{\nu,\mu}(t)\|^2_g \diff t .
% \end{equation} 
% \end{proposition}
\begin{theorem}[global optimality]\label{thm:global_optim}
The $\alpha$-geodesic $\gamma^{(\alpha)}$ describes curves that minimize the (global) $\alpha$-\emph{energy} $E^{(\alpha)}(\mu,\nu):=\frac{1}{p}\int_0^1 F^p(\gamma,\dot{\gamma}) \diff t$ among any smooth curve $\gamma$ connect $\mu$ to $\nu$.
\end{theorem}

\begin{corollary}
The 0-geodesic globally minimizes the curve length and the kinetic energy $\frac{1}{2}\int_0^1\|\dot{\gamma}\|_g^2\diff t$.
\end{corollary}

As the Fisher information metric coincides with the standard sphere metric for $\alpha=0$, the mapped geodesics are great circles on the sphere, leading to the following corollary:
\begin{corollary}\label{coro:sphere_geodesic}
For the vector field $u:=a/\sqrt{\mu}$ on the hypersphere, the curve that minimizes the kinetic energy $\frac{1}{2}\int_0^1 \|u_t\|^2_2\diff t=\frac{1}{2}\int_0^1 \|a_t\|^2_g\diff t$ between two points $x=\sqrt{\mu},y=\sqrt{\nu}$ is the great circle connecting $x$ and $y$.
\end{corollary}
\begin{corollary}
For two one-hot distributions $\delta_0,\delta_1$, the interpolation along the kinetic-energy minimizing curve adopts the following form:
\begin{equation}
    \mu_t=\delta_0\cos^2(t\pi/2)+\delta_1\sin^2(t\pi/2)
\end{equation}
\end{corollary}
The above corollaries coincide with the core results in \citet{shaul2024flow} and justify the usage of the cosine-squared scheduler $\kappa(t)=\cos^2(t\pi/2)$ in \citet{han2022ssd}.

\subsection{Classification of Continuous-State DFM Models}\label{sec:classification}
Following the conventions in information geometry, the ($-1$)-representation is called the $m$-representation ($m$ for mixture), and the 1-representation is called the $e$-representation ($e$ for exponential). Additionally, the $0$-geodesic corresponds to the Levi-Civita connection $\nabla^{(0)}$ and preserves the Fisher information metric. For general $\alpha$, the reparameterizations $\tau_{\mu,\nu},\tau_{\mu,a}$ do not have closed-form solutions. Nonetheless, the solutions for these three cases of $\alpha$-geodesics are known and have been explored in previous CS-DFM models. 
Despite our focus on continuous-state DFM, we note the potential of applying our $\alpha$-geodesics in discrete-state DFM and discrete diffusion models. For the latter, a probability path of categorical distributions also needs to be defined, on which the reverse diffusion process can be parameterized and learned by a neural net to stochastically convert initial tokens (often masks) to target tokens. 

\paragraph{Mixture class ($\alpha=-1$).} 
The $m$-geometry on the statistical manifold admits the linear embedding $\mu\mapsto \mu-1$ with a flat structure. The exponential and logarithm maps share the same formulae as the common Euclidean geometry:
\begin{align}
    \widetilde{\exp}^{(-1)}_x u&=x+u,\\
    \widetilde{\log}^{(-1)}_x y&=y-x.
\end{align}

We generally consider any model that operates linearly on the categorical probabilities (i.e., $m$-representations) as \emph{mixture-class}. This includes \emph{linear flow matching} used in previous work \cite{stark2024dirichlet,cheng2024categorical}, as it also assumes a flat Euclidean structure on the probabilities. The only difference is that the loss for linear flow matching uses the Euclidean norm $\|\cdot\|_2^2$ instead of the Riemannian norm $\|\cdot\|_g^2$. \citet{song2023equivariant,dunn2024mixed} used such linear models to generate discrete modality.
Furthermore, regarding DS-DFM and discrete diffusion models, most recent work \cite{sahoo2024simple,shi2024simplified,gat2024discrete} primarily adopted the $m$-geodesic as the interpolation path and can be, therefore, classified to the mixture class.


\paragraph{Metric class ($\alpha=0$).} 
The mapping $\pi^{(0)}$ projects categorical distributions onto the sphere $\mu\mapsto 2(\sqrt{\mu}-1)$, whose induced metric coincides with the inherited Euclidean metric (the canonical spherical geometry). Therefore, in this case, the $\alpha$-connection is the Levi-Civita connection that enjoys additional theoretical benefits mentioned in the previous theorems. With the spherical symmetry, the reparameterizations can be solved in closed form (see Appendix~\ref{supp:solve_geodesic}), leading to the canonical spherical geometry with the (mapped) $0$-geodesic being great circles on the sphere.

Two previous works \cite{cheng2024categorical,davis2024fisher} have explored such a canonical Riemannian structure on the statistical manifold of categorical distributions, following the spherical geodesics between the mapped representations of categorical distributions. Both papers also demonstrated the close relation of such a metric-class generative model to \emph{natural gradient} \cite{amari1998natural,amari1998adaptive}, the ``steepest'' direction of decreasing KL-divergence. As noted in Proposition \ref{prop:gradient}, a similar property holds for all $\alpha$-geodesic flows.
Additionally, in DS-DFM and discrete diffusion work, \citet{shaul2024flow} adopted a kinetic-optimal perspective to construct the path of categorical distributions. Adopting the canonical Fisher-information metric, \citet{shaul2024flow} arrived at precisely the same result as our Corollary \ref{coro:sphere_geodesic}, which is a special case of Theorem \ref{thm:local_optim} and \ref{thm:global_optim} establishing optimality for all $\alpha$-geodesic flows.
The usage of the corresponding scheduler (the cosine-squared scheduler) was proposed in \citet{han2022ssd} purely heuristically. Our results provide additional theoretical justifications.


\paragraph{Exponential class ($\alpha=1$).} 
The $e$-geometry on the statistical manifold admits an almost linear structure on the logit space with the logit mapping $\mu\mapsto\log\mu$. The exponential and logarithm maps can be calculated as
\begin{align}
    \widetilde{\exp}^{(1)}_x u&=x+u-\logsumexp(x+u),\label{eqn:log_exp} \\
    \widetilde{\log}^{(1)}_x y&=y-x+D_\text{KL}(\mu\|\nu).\label{eqn:log_log}
\end{align}

To the best of our knowledge, the above exponential-class exponential and logarithm maps have not been proposed in previous work. \citet{boll2024generative,boll2024generative2} explored a similar setting along the $e$-geodesic but used a different parameterization of the vector field without explicitly regressing the vector field with respect to Eq.\ref{eqn:log_log}.
Similar to the previous two classes, we generally consider any models operating on the logits (i.e., the $e$-representation up to the equivalence in the affine structure) as \emph{exponential-class}. In this sense, the earliest attempts at extending flow matching and diffusion models to discrete generative modeling can be considered. For example, \citet{hoogeboom2021argmax} assumes multiplicative noising of probabilities, therefore linearly operating in the logits space. \citet{mahabadi2023tess} performed diffusion on the logit space, and \citet{li2024full} adopted the linear flow matching on the logits for the discrete modality.
These existing models usually directly assume an underlying Euclidean structure on the logits without the additional correction term in Eq.\ref{eqn:log_exp} and \ref{eqn:log_log} as our rigorous formulation from information geometry.


==> tabs/bmnist.tex <==
\begin{table}[ht]
\centering
\vspace{-1em}
\caption{FID scores on the binarized MNIST dataset.}\label{tab:bmnist}
% \resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multirow{2}{*}{Model} & \multicolumn{6}{c}{CS-DFM} & \multicolumn{2}{c}{DS-DFM} \\ \cmidrule(l){2-7} \cmidrule(l){8-9} 
 & $\alpha=-1$ & $\alpha=-0.5$ & $\alpha=0$ & $\alpha=0.5$ & $\alpha=1$ & Linear & MDLM & DFM \\ \midrule
FID$\downarrow$ & 10.27 & 10.79 & \textbf{5.02} & 5.07 & 5.48 & 6.97 & 27.46 & 44.22 \\ \bottomrule
\end{tabular}
% }
\vspace{-0.5em}
\end{table}

==> tabs/swissroll.tex <==
\begin{table}[ht]
\centering
\vspace{-.5em}
\caption{KL divergence on the Swiss roll dataset.}\label{tab:swissroll}
% \resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
Model & $\alpha=-1$ & $\alpha=-0.5$ & $\alpha=0$ & $\alpha=0.5$ & $\alpha=1$ & Linear \\ \midrule
KLD$\downarrow$ & 1.617 & 0.485 & 0.637 & 0.905 & \textbf{0.476} & 0.583 \\ \bottomrule
\end{tabular}
% }
\vspace{-1.em}
\end{table}

==> tabs/text8.tex <==
\begin{table}[ht]
\centering
\vspace{-0.5em}
\caption{GPT-J-6B evaluated NLLs and generation entropy on Text8. The best is in \textbf{bold}, and the second best is \underline{underlined}. \textsuperscript{*} indicates results from \citet{campbell2024generative}.}\label{tab:text8}
\small
% \resizebox{\linewidth}{!}{
\begin{tabular}{@{}llccc@{}}
\toprule
Model Type & Model & NLL & Entropy & Entropy Diff \\ \midrule
\multirow{6}{*}{CS-DFM} & $\alpha=-1$ & 7.31 & 7.45 & \textbf{-0.03} \\
 & $\alpha=-0.5$ & 7.14 & 7.37 & -0.11 \\
 & $\alpha=0$ & 6.85 & 7.38 & -0.10 \\
 & $\alpha=0.5$ & 7.00 & 7.42 & {\ul -0.06} \\
 & $\alpha=1$ & 7.09 & 7.51 & \textbf{+0.03} \\
 & Linear & 7.35 & 7.62 & +0.14 \\ \midrule
 % & LogLinear & 6.81 & 7.34 & -0.14 \\ \midrule
\multirow{5}{*}{DS-DFM} & MDLM & 6.76 & 7.55 & +0.07 \\
 & DFM & 6.78 & 7.58 & +0.10 \\
 & D3PM[\citenum{austin2021structured}]\textsuperscript{*} & 6.93 & 7.38 & -0.10 \\
 & SEDD[\citenum{lou2023discrete}]\textsuperscript{*}& \textbf{6.49} & 7.17 & -0.31 \\
 & MultiFlow[\citenum{campbell2024generative}]\textsuperscript{*} & {\ul 6.73} & 7.39 & -0.09 \\ \midrule
 & Data\textsuperscript{*} & 4.10 & 7.48 & 0 \\ \bottomrule
\end{tabular}
% }
\vspace{-0.5em}
\end{table}


==> tabs/text8_sample.tex <==
\renewcommand{\arraystretch}{1.5}

\begin{table}[ht]
\centering
\small
\hspace*{2em}
\begin{tabular}{@{}l@{}}
$\alpha=-1$\\ 
\quad\begin{lstlisting}
n_the_gorisrisk_i_v_mit_k_one_nine_four_seven_one_nine_eight_six_flyzecag_rhylointius_gerland_franke_one_nine_six_six_costeananl
eloss_gubdrel_s_watches_s_orcusus_one_nine_seven_three_imanes_emz_four_nine_nuclear_waxetimes_mois_marrutus_prisstri_pet_sour_pe
\end{lstlisting}\\
\quad\begin{lstlisting}
cub_tobily_tractical_senior_animal_one_one_place_drier_thiaryja_sign_l_m_memorate_on_sweep_tmao_reformed_lights_of_one_five_one_
six_six_two_six_a_mijo_newark_espeeder_to_the_decries_of_gratgoy_coutoje_mortal_areas_decree_arizoni_royja_al_jad_rommri_al_the_
\end{lstlisting}\\
\quad\begin{lstlisting}
ped_oditors_in_the_early_two_zero_zero_zero_he_did_tr_nwarcoufes_bcp_sive_watchmitant_tabper_among_many_present_goes_appr_praiee
des_bbc_chandrei_congressons_cleeting_new_tract_two_rever_mitzes_congress_game_share_with_homelaustrists_clh_have_a_very_popular
\end{lstlisting}\\

$\alpha=-0.5$\\ 
\quad\begin{lstlisting}
g_at_the_movies_of_etropostone_and_as_the_force_all_from_canadian_new_nepal_in_november_one_nine_two_zero_the_sinonquitts_direct
ed_dr_ka_goddey_viewed_and_the_program_landed_worn_in_the_salash_republic_of_mone_steunsaudup_gt_hgp_was_decided_lo_sougoveen_br
\end{lstlisting}\\
\quad\begin{lstlisting}
five_one_three_st_michlen_j_james_cba_born_writer_d_one_nine_six_eight_one_nine_six_one_jemneur_meldemweril_akirak_caradishman_k
eveselkion_one_nine_eight_three_eonathy_todenlini_n_h_jeoreokh_vooyk_goga_american_actor_one_nine_six_one_riso_phillipp_p_nellan
\end{lstlisting}\\
\quad\begin{lstlisting}
l_apposes_to_the_sacrificing_yoster_ipice_stayed_to_be_someone_or_the_honors_of_gosrem_b_and_the_weening_and_hour_his_asserbly_i
n_jakinssen_to_proper_to_this_book_his_kirual_use_picea_studies_the_helm_to_laaseddate_themes_joan_flieta_took_from_the_kirk_s_m
\end{lstlisting}\\

$\alpha=0$\\ 
\quad\begin{lstlisting}
e_ipid_device_over_windows_the_in_virion_of_mvs_or_rvs_may_sqram_owners_on_documentary_flanes_in_detail_though_development_of_li
ving_is_aptertinacure_which_may_be_visually_detected_its_db_is_that_does_not_tell_information_about_the_intelliving_litgeon_info
\end{lstlisting}\\
\quad\begin{lstlisting}
_to_a_spvool_college_the_users_liked_to_add_popularly_as_do_mournables_against_manianes_often_relaid_on_be_used_to_delete_a_netb
reak_ruddhy_bestanding_of_alphabetian_examples_with_tunes_by_rome_and_calling_a_rebel_zene_against_the_prete_of_eras_the_rome_wa
\end{lstlisting}\\
\quad\begin{lstlisting}
two_the_appeal_assembly_has_an_encep_for_grants_t_a_statistical_productive_return_group_scheduled_to_pay_a_total_term_to_make_a_
relection_and_since_the_maghallo_constitution_is_ship_held_in_two_zero_zero_eight_which_includes_i_eleinnactes_ak_reprodaca_pecr
\end{lstlisting}\\

$\alpha=0.5$\\ 
\quad\begin{lstlisting}
e_majority_of_the_city_is_the_two_seyon_th_and_our_th_twh_of_the_populations_that_states_the_two_tetriarchs_three_members_of_the
_ird_council_known_as_the_city_the_irx_s_own_ipfn_government_in_the_decline_of_the_country_bastadgine_has_greatly_accedted_the_o
\end{lstlisting}\\
\quad\begin{lstlisting}
w_level_color_with_individuals_such_as_cork_lends_goods_that_take_bo_crami_that_is_ger_znney_corm_as_subsditial_substantial_poin
t_residency_is_formelated_with_the_urami_bo_karatac_mnddy_public_zones_tabri_the_share_of_new_banking_and_won_by_microeconomy_ba
\end{lstlisting}\\
\quad\begin{lstlisting}
ns_at_once_the_lackage_ennouraged_to_deliver_guiding_work_and_was_subdective_repressed_awricrn_americans_like_the_silichs_or_tha
t_it_call_federal_positions_that_are_view_and_aid_for_federal_in_africa_to_colony_as_it_was_said_that_joan_s_modern_member_noses
\end{lstlisting}\\

$\alpha=1$\\ 
\quad\begin{lstlisting}
_store_rolls_see_cord_statue_the_otches_in_the_doors_a_very_thin_attergace_the_unique_place_of_weak_the_world_bp_connected_to_bl
ack_any_certain_chance_you_wild_facilitate_on_the_pepae_the_chrovium_ion_was_known_to_launch_the_use_of_abards_crystosis_this_is
\end{lstlisting}\\
\quad\begin{lstlisting}
ained_the_talent_of_princeton_and_sholon_wubry_in_one_nine_nine_five_it_was_aeent_freeland_s_old_fyejider_that_bertrade_rydwar_o
f_j_doma_s_credit_and_was_redeted_to_university_stars_brad_john_if_sam_of_whom_he_asks_ofordos_the_princedom_wargirl_im_ako_in_h
\end{lstlisting}\\
\quad\begin{lstlisting}
atrix_from_which_long_history_and_swaeton_acts_as_the_pushtine_distance_that_sexually_oriented_you_the_themes_make_in_a_faccette
_the_junitune_a_conducting_event_and_can_be_sasily_inted_to_a_fycco_many_difficult_ill_round_it_living_non_hair_presents_a_lack_
\end{lstlisting}\\

Linear\\ 
\quad\begin{lstlisting}
_blnb_ff_he_has_survival_damaged_to_the_authority_would_move_a_prea_on_the_news_she_resources_but_pesh_to_heep_as_you_in_line_up
on_paras_pmetry_alight_a_interdict_with_on_the_cavers_published_and_continued_of_the_annx_reaking_in_rkisk_comic_stairek_vk_afte
\end{lstlisting}\\
\quad\begin{lstlisting}
name_mart_hoog_to_wear_this_list_of_reduncch_kranms_including_ceotroet_matrehiz_a_world_blue_that_crossed_according_to_his_pubs_
account_because_i_donot_believe_that_the_minnesoian_alphabet_wee_speaked_saw_an_effect_on_vochwaa_s_late_one_nine_five_zero_s_th
\end{lstlisting}\\
\quad\begin{lstlisting}
two_three_one_route_house_does_ad_region_above_ll_l_tabo_centre_two_four_the_topic_nomedous_is_s_six_zero_two_three_three_sereb_
nine_seven_seven_two_nine_rules_q_tiroides_lmatrime_uuf_additional_conscript_anti_air_coutl_sequences_contact_allowing_sto_to_do
\end{lstlisting}\\

MDLM\\ 
\quad\begin{lstlisting}
st_ii_papyrus_charles_biscaf_lowar_philippierre_aristotle_philosophers_man_s_influent_vassay_shaak_byzantine_emperor_hedwig_thos
paw_frank_k_sterossi_lawrent_ii_jordan_jakob_elow_fa_christian_weae_all_for_thomas_lucas_v_liel_kould_irena_georg_jo_wyhor_schol
\end{lstlisting}\\
\quad\begin{lstlisting}
hen_the_labor_cannot_lampey_when_any_through_the_trade_of_approach_when_value_is_read_and_percentiges_of_unemployed_price_when_t
he_wage_falls_come_in_position_checks_the_price_of_capitalism_whys_through_the_wages_that_contained_the_essence_of_these_the_sol
\end{lstlisting}\\
\quad\begin{lstlisting}
of_population_to_prolong_slave_labour_and_have_small_larger_sharpness_in_the_body_poof_height_populations_four_report_three_zero
_zero_netwees_among_grey_stones_trees_speedard_is_enlarged_by_the_passenger_to_rielling_small_needles_but_having_a_negative_spir
\end{lstlisting}\\

DFM\\ 
\quad\begin{lstlisting}
wo_n_property_of_evereygamma_o_gamma_n_neale_propertyodic_f_x_one_and_y_s_infty_d_x_b_x_one_n_n_x_infty_n_by_dic_one_x_one_m_n_s
ample_x_one_n_n_n_where_for_everex_q_one_one_y_m_real_inf_y_x_infry_int_g_d_x_y_m_not_real_time_weight_f_x_t_not_duple_q_phi_qui
\end{lstlisting}\\
\quad\begin{lstlisting}
earned_control_over_the_grand_hotel_by_the_council_of_state_to_produce_a_new_might_constat_the_only_personality_of_the_control_w
oman_s_personality_iv_the_tingereeur_for_the_state_the_does_not_goreon_school_is_hermetic_and_conservative_except_with_the_philo
\end{lstlisting}\\
\quad\begin{lstlisting}
gts_every_dc_series_which_features_bill_alice_lewis_is_mentioned_in_which_the_ducati_glore_s_main_character_s_sweet_formation_or
_the_murder_orderly_understopped_of_the_universe_the_character_of_the_dc_series_was_not_known_with_the_role_of_soviet_writer_dr_
\end{lstlisting}\\
\end{tabular}
\end{table}


